Beyond Linearization: On Quadratic and Higher-Order Approximation of Wide Neural Networks

Recent theoretical work has established connections between over-parametrized neural networks and linearized models governed by he Neural Tangent Kernels (NTKs). NTK theory leads to concrete convergence and generalization results, yet the empirical performance of neural networks are observed to exceed their linearized models, suggesting insufficiency of this theory. Towards closing this gap, we investigate the training of over-parametrized neural networks that are beyond the NTK regime yet still governed by the Taylor expansion of the network. We bring forward the idea of \emph{randomizing} the neural networks, which allows them to escape their NTK and couple with quadratic models. We show that the optimization landscape of randomized two-layer networks are nice and amenable to escaping-saddle algorithms. We prove concrete generalization and expressivity results on these randomized networks, which lead to sample complexity bounds (of learning certain simple functions) that match the NTK and can in addition be better by a dimension factor when mild distributional assumptions are present. We demonstrate that our randomization technique can be generalized systematically beyond the quadratic case, by using it to find networks that are coupled with higher-order terms in their Taylor series.

==> Sections_iclr_revision/higher-ntk.tex <==
\section{Higher-order NTKs}
\label{section:higher-order}
We demonstrate that our idea of randomization for
changing the dynamics of learning neural networks can be generalized
systematically --- through randomization we are able to obtain
over-parametrized neural networks in which the $k$-th order term
dominates the Taylor series. Due to space constraints, we provide our
concrete results on the coupling, generalization, and expressivity of
higher-order models in Appendix~\ref{appendix:higher-ntk-gen}.

% \yub{Below to be removed.}

% In this section, we demonstrate that our idea of randomization for
% changing the dynamics of learning neural networks can be generalized
% systematically --- through randomization we are able to obtain
% over-parametrized neural networks in which the $k$-th order term
% dominates the Taylor series.  Consider a two-layer neural network with
% $2m$ neurons and symmetric initialization
% (cf.~\eqref{equation:symmetric-init})
% \begin{equation*}
%   f_{\bW_0+\bW}(\bx) = \frac{1}{\sqrt{m}}\sum_{r\le m}
%   \sigma((\bw_{0,r}+\bw_{+,r})^\top\bx) -
%   \sigma((\bw_{0,r}+\bw_{-,r})^\top\bx).
% \end{equation*}
% Assuming $\sigma$ is analytic on $\R$ (i.e. it equals its Taylor
% series at any point), we have
% % \begin{equation*}
% $
% f_{\bW_0+\bW}(\bx) = \sum_{k=0}^\infty f^{(k)}_{\bW_0,\bW}(\bx),
% $
% % \end{equation*}
% where we have defined the \emph{$k$-th order NTK}
% \begin{equation*}
%   f^{(k)}_{\bW_0, \bW}(\bx) \defeq \frac{1}{\sqrt{m}}\sum_{r\le m}
%   \frac{1}{k!} \sigma^{(k)}(\bw_{0,r}^\top\bx)
%   \paren{(\bw_{+,r}^\top\bx)^k - (\bw_{-,r}^\top\bx)^k}.
% \end{equation*}
% Note that $f^{(0)}(\bx)\equiv 0$ due to the symmetric initialization,
% and $f^{(1)}(\bx)$ is the standard NTK.

% % \vspace{-0.2cm} 
% \paragraph{Coupling with $f^{(k)}$ via randomization}
% We show in Appendix~\ref{appendix:higher-ntk-coupling} that for any
% $k\ge 2$, there exists a randomized $\bW$ at which
% $f_{\bW_0+\bW}(\bx) = f^{(k)}_{\bW_0,\bW}(\bx) + o_m(1)$. More
% concretely, our choice of $\bW$ is such that all of
% $f^{(1)},\dots,f^{(k-1)}$ have on average $o_m(1)$ in magnitude, and
% $f^{(k)}=O(1)$ is the dominating term.

% % \vspace{-0.2cm}
% % \paragraph{Generalization, expressivity, and ``deterministic''
% % coupling}
% \paragraph{Generalization and expressivity}
% We establish the generalization of expressivity of $f^{(k)}$ in
% Appendix~\ref{appendix:higher-ntk-gen-expressivity}, which
% systematically extends
% our results on the quadratic model. We show that the sample complexity
% for learning degree $\ge k$ polynomials through $f^{(k)}$ compared
% with linear NTK can be better by a factor of $d^{k-1}$ for large $n$,
% when mild distributional assumptions on $\bx$ such as approximate isotropy (constant condition number of the $k^{th}$ moment tensor) is present.

% \paragraph{Existence through concentration}
% Further, one can extend the concentration arguments on the above randomization to show the existence of some deterministic) $\bW$ at which the neural net is approximately the $k$-th order NTK: $\E_{\bx}[|f_{\bW_0+\bW}(\bx) - f^{(k)}_{\bW_0,\bW}(\bx)|]\le \eps_m$,
% where $\eps_m\to 0$ as $m\to\infty$. We would like to leave this as future work.

% Using the probabilistic method, there exists one such
% choice of $\set{z_{+,r},z_{-,r}}_{r\le m}$, under which the above
% statement determinstically holds.

% \subsection{Expressivity}

% \subsection{Generalization}


==> Sections_iclr_revision/opt-clean.tex <==
\section{Optimization}
\subsection{Clean risk}

